Free Gap Information from the Differentially Private Sparse Vector and Noisy Max Mechanisms

Noisy Max and Sparse Vector are selection algorithms for differential privacy and serve as building blocks for more complex algorithms. In this paper we show that both algorithms can release additional information for free (i.e., at no additional privacy cost). Noisy Max is used to return the approximate maximizer among a set of queries. We show that it can also release for free the noisy gap between the approximate maximizer and runner-up. This free information can improve the accuracy of certain subsequent counting queries by up to 50%. Sparse Vector is used to return a set of queries that are approximately larger than a fixed threshold. We show that it can adaptively control its privacy budget (use less budget for queries that are likely to be much larger than the threshold) in order to increase the amount of queries it can process. These results follow from a careful privacy analysis.

==> proof_adaptsvt.tex <==
We prove the Lemma using the following two results
\begin{lemma}\label{lem:local_adaptivesvt_align}
Let $M$ be the \adaptivesvt algorithm.
For all $D\sim D^\prime$ and $\omega$, the functions $\alio$ defined by \eqref{eq:adaptivesvt_align} are local alignments for $M$. 
%That is, if $M(D,H)=\omega$ then $M(D^\prime, \alio(H))=\omega$. 
Furthermore, for every pair $D\sim D^\prime$, there are countably many distinct $\alio$.
\end{lemma}


\begin{proof}
First note that $\alio$ only depends on $\omega$ through $\io$ and $\jo$ (the sets of queries whose noisy values were larger than the noisy threshold). Since $\abs{\io}\leq k$ and $\abs{\jo}\leq k$, there are only countably many possibilities for $\io$ and $\jo$, hence there are countably many distinct $\alio$.

Pick an adjacent pair $D\sim D^\prime$ and an $\omega=(\omega_1,\dots,\omega_s)$.
For a given $H=(\eta, \xi_1,\eta_1,\dots)$ such that $M(D,H)=\omega$, let $H^\prime=(\eta^\prime,\xi_1^\prime, \eta_1^\prime, \dots) = \alio(H)$.

Let $M(D',H') = \omega' =(w_1', \ldots, w_{t}')$. Our goal is to show $\omega^\prime=\omega$. Choose an $i\leq \min(s,t)$. 
\begin{itemize}[leftmargin=0.5cm,itemsep=0cm,topsep=0.5em,parsep=0.5em]
    \item If $i\in\cI_\omega$, then by \eqref{eq:adaptivesvt_align} we have
\begin{align*}
    q_i' &+ \xi_i' - (T + \eta') = q_i' + \xi_i + 1 + q_i - q_i' - (T + \eta + 1) \\
    & = q_i + \xi_i -(T+\eta)  \geq \sigma.
\end{align*}
Therefore, $w_i' = w_i$.

\item If $i\in\cJ_\omega$, then by \eqref{eq:adaptivesvt_align} we have
\begin{align*}
    q_i' &+ \xi_i' - (T + \eta') = q_i' + \xi_i  - (T + \eta + 1) \\
    & = q_i' - 1 + \xi_i -(T+\eta) \leq q_i + \xi_i - (T+\eta) < \sigma\\
    q_i' &+ \eta_i' - (T + \eta') = q_i' +\eta_i + 1 + q_i - q_i'  - (T + \eta + 1) \\
    &=  q_i + \eta_i - (T+\eta)  \geq 0
\end{align*}
The first inequality is due to the sensitivity restriction: $\abs{q_i-q_i'}\leq 1 \implies q_i'-1\leq q_i$.
Hence $w_i' =  w_i$.
\item If $i\not\in \cI_\omega\cup\cJ_\omega$, then by a similar argument we have 
\begin{align*}
    q_i' + \xi_i' - (T + \eta') &\leq q_i + \eta_i - (T+\eta) < \sigma,\\
    q_i' + \eta_i' - (T + \eta') &\leq q_i + \xi_i - (T+\eta) < 0.
\end{align*}
Hence $w_i' = (\bot, 0) = w_i$.
\end{itemize}
Therefore, either $\omega'$ is a prefix of $\omega$ or vice versa. By a similar argument on the termination condition as before, we must have $s=t$ and thus $\omega' = \omega$. 
\end{proof}

\begin{lemma}\label{lem:local_adaptivesvt_cost}
Algorithm \ref{alg:adaptivesvt} satisfies $\epsilon$-differential privacy. %If $\vq$ is monotonic (Definition \ref{def:mono}), then Algorithm \ref{alg:gaptopk} satisfies $\epsilon/2$-differential privacy.
\end{lemma}
\begin{proof}
Again, the only thing nontrivial is to show that Condition (iv) of Lemma \ref{lem:alignmentbound} holds. The local alignments are clearly acyclic. To find their cost, we use the $\epsilon_0, \epsilon_1, \epsilon_2$ and $\epsilon$ defined in Algorithm \ref{alg:adaptivesvt}. 
From \eqref{eq:adaptivesvt_align} we have 
\begin{align*}
\cost(\alio) &=\epsilon_0\abs{\eta'-\eta} + \sum_{i=1}^\infty \epsilon_1\abs{\xi_i'-\xi_i} + \epsilon_2\abs{\eta_i'-\eta_i}\\
&= \epsilon_0 + \sum_{i\in \cI_\omega} \epsilon_1\abs{1 + q_i - q_i'} + \sum_{i\in \cJ_\omega} \epsilon_2\abs{1 + q_i - q_i'} \\
&\leq  \epsilon_0 + 2\epsilon_1\abs{\cI_\omega} + 2\epsilon_2\abs{\cJ_\omega} \leq \epsilon.
\end{align*}
The first inequality is from sensitivity assumption. The second inequality is from loop invariant: $\epsilon_0 + 2\epsilon_1\abs{\cI_\omega} + 2\epsilon_2\abs{\cJ_\omega} =\mathtt{cost} \leq \epsilon - 2\epsilon_2 + \max(2\epsilon_1, 2\epsilon_2) = \epsilon$.
\end{proof}
The proof of Lemma \ref{lem:adaptivesvt} now follows from Lemmas \ref{lem:local_adaptivesvt_align} and \ref{lem:local_adaptivesvt_cost}.

==> subsec_gapsvt.tex <==
As a warmup demonstration of the power of Lemma \ref{lem:alignmentbound}, we provide the first human-readable proof of \gapsvt~\cite{shadowdp}.
\begin{algorithm}[ht]
\SetKwProg{Fn}{function}{\string:}{}
\SetKwFunction{Test}{\funcsvt}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\DontPrintSemicolon
\Input{$\vq$: a list of queries of global sensitivity 1 \\
$D$: database, $\epsilon$: privacy budget, $T$: threshold\\
$k$: bound on above-$T$ answers to output}
\Fn{\Test{$\vq$, $D$, $T$, $k$, $\epsilon$}}{
$\epsilon_0 \gets \epsilon / 2$; $\epsilon_1 \gets \epsilon / (4k)$; $\mathtt{count} \gets 0$\;
$\eta \gets \lap(1/\epsilon_0)$\;
$\widetilde{T} \gets T + \eta$\;
\ForEach{$\mathtt{i} \in \set{1, \cdots, \len(\vq)}$}{
$\eta_i \gets \lap(1/\epsilon_1)$\;
\eIf{$q_i(D) + \eta_i - \widetilde{T} \geq 0$\label{line:gapsvt_noise}}
{
%\fbox{$\begin{cases} \Output{\texttt{true}} & \\ \Output{(q_i(D)+\eta_i-\tilde{T})} & \end{cases}$\;\label{line:gapsvt_out}}
\textbf{output:} $\top$, \fbox{$\mathtt{gap}=(q_i(D)+\eta_i-\widetilde{T})$}\label{line:gapsvt_out}\;
$\mathtt{count} \gets \mathtt{count} + 1$\;
}
{
\textbf{output:} $\bot$}\label{line:svt_out}
\lIf{$\mathtt{count} \ge k$}{\textbf{break}}
}
}
\caption{Sparse Vector (with Gap \protect\cite{shadowdp}). For the original SVT \protect\cite{diffpbook,lyu2017understanding}, remove the box on Line \ref{line:gapsvt_out}.}
\label{alg:svt}
\end{algorithm}
%
 The mechanism of Wang et al. \cite{shadowdp} is an improvement over the original Sparse Vector Technique (SVT) \cite{Dwork09STOCOnTheComplexity,Hardt2010svt} (providing strictly more information at the same privacy cost). The original SVT is a differentially private mechanism whose input is a sequence of queries with sensitivity 1. It estimates the identities of the first $k$ queries whose values are over a public threshold $T$. The original mechanism adds noise to the threshold and to each query. Then as it processes the queries in order, it returns $\top$ if the noisy query is above the noisy threshold and $\perp$ if it is below. It stops after outputting $\top$ for $k$ times. Wang et al. \cite{shadowdp} showed that in addition to outputting $\top$, it can also output \emph{at no extra cost to privacy} an estimate of the gap between the noisy query (for which $\top$ was produced) and the noisy threshold. Both versions of the mechanism are shown in Algorithm~\ref{alg:svt}, with the changes proposed by Wang et al. \cite{shadowdp} appearing in the box on line \ref{line:gapsvt_out} (note it re-uses the same noise as Line \ref{line:gapsvt_noise}).

Wang et al. \cite{shadowdp} verified the correctness of this mechanism using novel program verification techniques based on a complex type system; this method could not produce a human-readable proof. Lemma \ref{lem:alignmentbound} can be easily used to prove the correctness by simply specifying a set of local alignments.

%In \cite{shadowdp} Wang et al. proposed and verified a novel variant called \gapsvt that releases the gap between noisy over-threshold queries and the noisy threshold. The only difference is Line~\ref{line:gapsvt_out} of Algorithm~\ref{alg:svt} in which \svt outputs \texttt{true} whereas \gapsvt outputs the numeric gap. In this section, we provide the first human-readable proof for \gapsvt.


%\textbf{The setting} Let $Q=(Q_1, \ldots, Q_n)$ be a list of numerical queries of sensitivity 1, that is, $\forall D\sim D', ~\abs{Q_i(D)-Q_i(D')}\leq 1$.  For simplicity we write $q_i=Q_i(D)$ and $q'_i=Q_i(D')$. Let $T$ be a threshold and $c$ is an upper bound on the number of above-threshold queries to return.  Let $H$ denote the random variables used by $M$.

\paragraph*{Local alignment}
To create a local alignment for each $D\sim D^\prime$, first let $H=(\eta, \eta_1,\eta_2,\dots)$ where $\eta$ is the noise added to threshold $T$ and $\eta_i$ is the noise that should be added to the $i^\text{th}$ query $q_i$ (if execution ever reaches that point). We view the output $\omega=(\omega_1,\dots,\omega_s)$ as a variable-length sequence where each $\omega_i$ is either $\perp$ or the nonnegative gap (we omit the $\top$ as it is redundant). 

Let $\mathcal{I}_\omega=\set{i\mid w_i\in\RR^{\geq 0}}$. It is the index set of over-threshold queries (i.e. the ones for which a gap is returned). For $H\in \sdo$ (see notation in Table \ref{tab:notation}), define
$\alio(H)=H'=(\eta',\eta_1',\eta'_2,\ldots)$ where
\begin{equation}\label{eq:alignGapSvt}
    \eta' = \eta + 1,\quad
    \eta_i' =\begin{cases}
\eta_i + (1 +q_i(D) -q_i(D^\prime)), &i \in\mathcal{I}_\omega\\
\eta_i, &i \not\in\mathcal{I}_\omega
\end{cases}
\end{equation}
That is, to make sure $M(D^\prime,H^\prime)$ returns the same output as $M(D, H)$, we increase by one the noise added to the threshold ($\eta^\prime=\eta+1$) while keeping the noise added to below-threshold queries the same (hence if $q_i(D)+\eta_i$ is less than $T+\eta$ then  $q_i(D^\prime)+\eta^\prime_i$ is less than $T+\eta^\prime$). To make sure the over-threshold queries $q_j$ remain above the threshold with the same gap, we need to modify the noise $\eta_j^\prime$ so that $q_j(D)+\eta_j - (T+\eta) = q_j(D^\prime)+\eta_j^\prime - (T+\eta^\prime)$. Solving for $\eta_j^\prime$ gives us Equation \ref{eq:alignGapSvt}.

%That is, the threshold noise increases by $1$, and the noise for each query increases by $1 +q_i(D) -q_i(D^\prime)$ if the query is above threshold, or remains the same if the query is below threshold or is not processed (program already halted).

\begin{lemma}\label{lem:svtgap_align}
Let $M$ be the \gapsvt mechanism.
For all $D\sim D^\prime$ and $\omega$, the functions $\alio$ defined above are local alignments for $M$. That is, if $M(D,H)=\omega$ then $M(D^\prime, \alio(H))=\omega$. Furthermore, for every pair $D\sim D^\prime$, there are countably many distinct $\alio$.
\end{lemma}

The proof can be found in the \appendixref.
%the full version of this paper \cite{freegapinfo}. 
Once the local alignment has been constructed, we can use Lemma \ref{lem:alignmentbound} to prove privacy as follows.

\begin{lemma}\label{lem:costsvt}
Algorithm \ref{alg:svt} satisfies $\epsilon$-differential privacy.
\end{lemma}
\begin{proof}
Let $M$ be the mechanism. The $\alio$ are local alignments by Lemma \ref{lem:svtgap_align}. Clearly $M$ terminates with probability 1 (Condition (i) of the Lemma \ref{lem:alignmentbound}). The number of random variables used by $M$ is 1 + the length of the output. Hence Condition (ii) is satisfied. Condition (iii) is trivial and Condition (v) follows from Lemma \ref{lem:svtgap_align}. The only thing left to show is that Condition (iv) holds. Clearly the local alignments are acyclic. To find their cost, we use the $\epsilon_0, \epsilon_1, $ and $\epsilon$ defined in Algorithm \ref{alg:svt}.
\begin{align*}
\abs{\eta'-\eta}\epsilon_0 &+ \sum_{i=1}^n \abs{\eta_i'-\eta_i}\epsilon_1= \epsilon_0 +  \sum_{i\in\cI_\omega}\abs{1+ q_i(D)-q_i(D^\prime)}\epsilon_1  \\
&\leq \epsilon_0 + \sum_{i\in\cI_\omega} 2\epsilon_1 = \frac{\epsilon}{2} + 2\cdot \frac{\epsilon}{4k}\cdot \abs{\mathcal{I}_\omega}\leq \epsilon.
\end{align*}
The first inequality follows from the triangle inequality and sensitivity 1 of the queries: $\abs{1+q_i(D)-q_i(D')}\leq 1+ \abs{q_i(D)-q_i(D')} \leq 2$. The second inequality follows from the fact that there are at most $k$ above-the-threshold queries answered so $\abs{\cI_\omega}\leq k$. Thus all local alignments have cost $\leq \epsilon$.
\end{proof}

